A geometric characterization of the classical Lie algebras

A nonzero element x in a Lie algebra g over a field F with Lie product [ , ] is called a extremal element if [x, [x, g]] is contained in Fx. Long root elements in classical Lie algebras are examples of extremal elements. Arjeh Cohen et al. initiated the investigation of Lie algebras generated by extremal elements in order to provide a geometric characterization of the classical Lie algebras generated by their long root el- ements. He and Gabor Ivanyos studied the so-called extremal geometry with as points the 1-dimensional subspaces of g generated by extremal elements of g and as lines the 2-dimensional subspaces of g all whose nonzero vectors are extremal. For simple finite dimensional g this geometry turns out to be a root shadow space of a spherical building. In this paper we show that the isomorphism type of g is determined by its extremal geometry, provided the building has rank at least 3.

==> Bibliography8.tex <==

\begin{bibdiv}
\begin{biblist}




\bib{Ben74}{book}{
   author={Benkart, Georgia McClure},
   title={Inner ideals and the structure of Lie algebras},
   note={Thesis (Ph.D.)--Yale University},
   publisher={ProQuest LLC, Ann Arbor, MI},
   date={1974},
   pages={119},
   %review={\MR{2625003}},
}


\bib{Ben76}{article}{
   author={Benkart, Georgia},
   title={The Lie inner ideal structure of associative rings},
   journal={J. Algebra},
   volume={43},
   date={1976},
   number={2},
   pages={561--584},
   issn={0021-8693},
   %review={\MR{0435149 (55 \#8110)}},
}
\bib{Ben77}{article}{
   author={Benkart, Georgia},
   title={On inner ideals and ad-nilpotent elements of Lie algebras},
   journal={Trans. Amer. Math. Soc.},
   volume={232},
   date={1977},
   pages={61--81},
   issn={0002-9947},
   %review={\MR{0466242 (57 \#6122)}},
}
\bib{Blo11}{article}{
   author={Blok, R. J.},
   title={Highest weight modules and polarized embeddings of shadow spaces},
   journal={J. Algebraic Combin.},
   volume={34},
   date={2011},
   number={1},
   pages={67--113},
   issn={0925-9899},
   %review={\MR{2805201 (2012e:20100)}},
   %doi={10.1007/s10801-010-0263-3},
}		



\bib{BP03}{article}{
   author={Blok, R. J.},
   author={Pasini, A.},
   title={On absolutely universal embeddings},
   note={Combinatorics 2000 (Gaeta)},
   journal={Discrete Math.},
   volume={267},
   date={2003},
   number={1-3},
   pages={45--62},
   issn={0012-365X},
   %review={\MR{1991561 (2004f:51017)}},
}




\bib{BS02}{article}{
   author={Baranov, A. A.},
   author={Strade, H.},
   title={Finitary Lie algebras},
   journal={J. Algebra},
   volume={254},
   date={2002},
   number={1},
   pages={173--211},
   issn={0021-8693},
   %review={\MR{1927437 (2003g:17012)}},
   %doi={10.1016/S0021-8693(02)00079-0},
}
   

\bib{Bou68}{book}{
   author={Bourbaki, N.},
   title={\'El\'ements de math\'ematique. Fasc. XXXIV. Groupes et alg\`ebres
   de Lie. Chapitre IV: Groupes de Coxeter et syst\`emes de Tits. Chapitre
   V: Groupes engendr\'es par des r\'eflexions. Chapitre VI: syst\`emes de
   racines},
   language={French},
   series={Actualit\'es Scientifiques et Industrielles, No. 1337},
   publisher={Hermann, Paris},
   date={1968},
   pages={288 pp. (loose errata)},
   %review={\MR{0240238 (39 \#1590)}},
}

\bib{BC13}{book}{
   author={Buekenhout, F.},
   author={Cohen, A. M.},
   title={Diagram geometry},
   series={Ergebnisse der Mathematik und ihrer Grenzgebiete. 3. Folge. A
   Series of Modern Surveys in Mathematics [Results in Mathematics and
   Related Areas. 3rd Series. A Series of Modern Surveys in Mathematics]},
   volume={57},
   note={Related to classical groups and buildings},
   publisher={Springer, Heidelberg},
   date={2013},
   pages={xiv+592},
   isbn={978-3-642-34452-7},
   isbn={978-3-642-34453-4},
   %review={\MR{3014979}},
   %doi={10.1007/978-3-642-34453-4},
}
\bib{BS74}{article}{
   author={Buekenhout, Francis},
   author={Shult, Ernest},
   title={On the foundations of polar geometry},
   journal={Geometriae Dedicata},
   volume={3},
   date={1974},
   pages={155--170},
   issn={0046-5755},
   %review={\MR{0350599 (50 \#3091)}},
}
		


	
\bib{Car72}{book}{
   author={Carter, Roger W.},
   title={Simple groups of Lie type},
   note={Pure and Applied Mathematics, Vol. 28},
   publisher={John Wiley \& Sons, London-New York-Sydney},
   date={1972},
   pages={viii+331},
   %review={\MR{0407163 (53 \#10946)}},
}
\bib{CCS99}{article}{
   author={Cohen, A. M.},
   author={Cuypers, H.},
   author={Sterk, H.},
   title={Linear groups generated by reflection tori},
   note={Dedicated to H. S. M. Coxeter on the occasion of his 90th
   birthday},
   journal={Canad. J. Math.},
   volume={51},
   date={1999},
   number={6},
   pages={1149--1174},
   issn={0008-414X},
   %review={\MR{1756876 (2001e:20038)}},
   %doi={10.4153/CJM-1999-051-7},
}


\bib{Che89}{article}{
   author={Chernousov, V. I.},
   title={The Hasse principle for groups of type $E_8$},
   language={Russian},
   journal={Dokl. Akad. Nauk SSSR},
   volume={306},
   date={1989},
   number={5},
   pages={1059--1063},
   issn={0002-3264},
   translation={
      journal={Soviet Math. Dokl.},
      volume={39},
      date={1989},
      number={3},
      pages={592--596},
      issn={0197-6788},
   },
   %review={\MR{1014762 (90m:11055)}},
}
\bib{CI06}{article}{
   author={Cohen, A. M.},
   author={Ivanyos, G.},
   title={Root filtration spaces from Lie algebras and abstract root groups},
   journal={J. Algebra},
   volume={300},
   date={2006},
   number={2},
   pages={433--454},
   issn={0021-8693},
   %review={\MR{2228205 (2008a:17008)}},
   %doi={10.1016/j.jalgebra.2005.09.043},
}
\bib{CI07}{article}{
   author={Cohen, A. M.},
   author={Ivanyos, G.},
   title={Root shadow spaces},
   journal={European J. Combin.},
   volume={28},
   date={2007},
   number={5},
   pages={1419--1441},
   issn={0195-6698},
   %review={\MR{2320071 (2008e:20043)}},
   %doi={10.1016/j.ejc.2006.05.016},
}
\bib{CIR08}{article}{
   author={Cohen, A. M.},
   author={Ivanyos, G.},
   author={Roozemond, D.},
   title={Simple Lie algebras having extremal elements},
   journal={Indag. Math. (N.S.)},
   volume={19},
   date={2008},
   number={2},
   pages={177--188},
   issn={0019-3577},
   %review={\MR{2489325 (2010d:17012)}},
   %doi={10.1016/S0019-3577(09)00003-2},
}
\bib{CSUW01}{article}{
   author={Cohen, A. M.},
   author={Steinbach, A.},
   author={Ushirobira, R.},
   author={Wales, D.},
   title={Lie algebras generated by extremal elements},
   journal={J. Algebra},
   volume={236},
   date={2001},
   number={1},
   pages={122--154},
   issn={0021-8693},
   %review={\MR{1808349 (2001k:17007)}},
   %doi={10.1006/jabr.2000.8508},
}

\bib{Coh12}{article}{
   author={Cohen, A. M.},
   title={The geometry of extremal elements in a Lie algebra},
   conference={
      title={Buildings, finite geometries and groups},
   },
   book={
      series={Springer Proc. Math.},
      volume={10},
      publisher={Springer, New York},
   },
   date={2012},
   pages={15--35},
   %review={\MR{3074860}},
   %doi={10.1007/978-1-4614-0709-6-2},
}
\bib{Coh}{book}{
   author={Cohen, A. M.},
   title={Diagram Geometry, Related to Lie algebras and exceptional groups},
   series={ available at www.win.tue.nl/$\sim$amc/buek/book2.pdf},
   volume={},
   note={},
   publisher={preliminary version 2014},
   date={},
   pages={},
   isbn={},
   %review={},
}

%\bib{CJP92}{article}{
%   author={Cuypers, Hans},
%   author={Johnson, Peter},
%   author={Pasini, Antonio},
%   title={On the embeddability of polar spaces},
%   journal={Geom. Dedicata},
%   volume={44},
%   date={1992},
%   number={3},
%   pages={349--358},
%   issn={0046-5755},
%   %review={\MR{1193124 (94f:51008)}},
%   %doi={10.1007/BF00181400},
%}
\bib{CJP93}{article}{
   author={Cuypers, H.},
   author={Johnson, P.},
   author={Pasini, A.},
   title={On the classification of polar spaces},
   journal={J. Geom.},
   volume={48},
   date={1993},
   number={1-2},
   pages={56--62},
   issn={0047-2468},
   %review={\MR{1242702 (94h:51007)}},
   %doi={10.1007/BF01226800},
}
		


 
\bib{Cuy91}{article}{
   author={Cuypers, H.},
   title={Symplectic geometries, transvection groups, and modules},
   journal={J. Combin. Theory Ser. A},
   volume={65},
   date={1994},
   number={1},
   pages={39--59},
   issn={0097-3165},
   %review={\MR{1255262 (94m:51003)}},
   %doi={10.1016/0097-3165(94)90036-1},
}
 \bib{CRS14}{article}{
   author={Cuypers, H.},
   author={Roberts, K.},
   author={Shpectorov, S.},
   title={Recovering the Lie algebra from its extremal geometry},
   journal={J. Algebra},
   volume={441},
   date={2015},
   pages={196--215},
   issn={0021-8693},
   %review={\MR{3391926}},
   %doi={10.1016/j.jalgebra.2015.06.037},
}
\bib{cuyfle}{article}{
   author={Cuypers, H.},
   author={Fleischmann, Y.},
   title={A geometric characterization of the symplectic Lie algebra },
   date={2017},
}


\bib{Dip08}{article}{
   author={Draisma, J.},
   author={in 't panhuis, J.},
   title={Constructing simply laced Lie algebras from extremal elements},
   journal={Algebra Number Theory},
   volume={2},
   date={2008},
   number={5},
   pages={551--572},
   issn={1937-0652},
   %review={\MR{2429453 (2009e:17012)}},
   %doi={10.2140/ant.2008.2.551},
}

\bib{Fau73}{article}{
   author={Faulkner, J. R.},
   title={On the geometry of inner ideals},
   journal={J. Algebra},
   volume={26},
   date={1973},
   pages={1--9},
   issn={0021-8693},
   %review={\MR{0367002 (51 \#3247)}},
}

\bib{Fis71}{article}{
   author={Fischer, B.},
   title={Finite groups generated by $3$-transpositions. I},
   journal={Invent. Math.},
   volume={13},
   date={1971},
   pages={232--246},
   issn={0020-9910},
   %review={\MR{0294487 (45 \#3557)}},
}
		
\bib{fle15}{book}{
   author={Fleischmann, Y.},
   title={A Geometric Approach to Classical Lie Algebras},
   school={PhD thesis, Technische Universiteit Eindhoven},
   date={2015},
}

\bib{deGr00}{book}{
   author={de Graaf, W. A.},
   title={Lie algebras: theory and algorithms},
   series={North-Holland Mathematical Library},
   volume={56},
   publisher={North-Holland Publishing Co., Amsterdam},
   date={2000},
   pages={xii+393},
   isbn={0-444-50116-9},
   %review={\MR{1743970 (2001j:17011)}},
   %doi={10.1016/S0924-6509(00)80040-9},
}

\bib{Hal94}{article}{
   author={Hall, J. I.},
   title={Locally finite simple groups of finitary linear transformations},
   conference={
      title={Finite and locally finite groups},
      address={Istanbul},
      date={1994},
   },
   book={
      series={NATO Adv. Sci. Inst. Ser. C Math. Phys. Sci.},
      volume={471},
      publisher={Kluwer Acad. Publ., Dordrecht},
   },
   date={1995},
   pages={147--188},
   %review={\MR{1362809 (96j:20042)}},
   %doi={10.1007/978-94-011-0329-96},
}

\bib{Hog82}{article}{
   author={Hogeweij, G. M. D.},
   title={Almost-classical Lie algebras. I, II},
   journal={Nederl. Akad. Wetensch. Indag. Math.},
   volume={44},
   date={1982},
   number={4},
   pages={441--452, 453--460},
   issn={0019-3577},
   %review={\MR{683531 (84f:17007)}},
}
\bib{Hum72}{book}{
   author={Humphreys, James E.},
   title={Introduction to Lie algebras and representation theory},
   series={Graduate Texts in Mathematics},
   volume={9},
   note={Second printing, revised},
   publisher={Springer-Verlag, New York-Berlin},
   date={1978},
   pages={xii+171},
   isbn={0-387-90053-5},
   %review={\MR{499562 (81b:17007)}},
}
\bib{itp09}{book}{
   author={in 't panhuis, J.},
   title={ Lie algebras, extremal elements, and geometries},
   school={PhD thesis, Technische Universiteit Eindhoven},
   date={2009},
}
\bib{itpPR09}{article}{
   author={in 't panhuis, J.},
   author={Postma, E.},
   author={Roozemond, D.},
   title={Extremal presentations for classical Lie algebras},
   journal={J. Algebra},
   volume={322},
   date={2009},
   number={2},
   pages={295--326},
   issn={0021-8693},
   %review={\MR{2529091 (2010d:17008)}},
   %doi={10.1016/j.jalgebra.2009.04.015},
}
\bib{Jac79}{book}{
   author={Jacobson, Nathan},
   title={Lie algebras},
   note={Republication of the 1962 original},
   publisher={Dover Publications, Inc., New York},
   date={1979},
   pages={ix+331},
   isbn={0-486-63832-4},
   %review={\MR{559927 (80k:17001)}},
}
\bib{Joh90}{article}{
   author={Johnson, Peter M.},
   title={Polar spaces of arbitrary rank},
   journal={Geom. Dedicata},
   volume={35},
   date={1990},
   number={1-3},
   pages={229--250},
   issn={0046-5755},
   %review={\MR{1066567 (91i:51006)}},
   %doi={10.1007/BF00147348},
}
\bib{KS01}{article}{
   author={Kasikova, A.},
   author={Shult, E.},
   title={Absolute embeddings of point-line geometries},
   journal={J. Algebra},
   volume={238},
   date={2001},
   number={1},
   pages={265--291},
   issn={0021-8693},
   %review={\MR{1822192 (2003a:51014)}},
   %doi={10.1006/jabr.2000.8629},
}
ISSN 2167-5163
\bib{Pos07}{book}{
   author={Postma, Erik},
   title={From Lie Algebras to Geometry and Back},
   school={PhD thesis, Technische Universiteit Eindhoven},
   date={2007},
}


\bib{Pre86-1}{article}{
   author={Premet, A. A.},
   title={Inner ideals in modular Lie algebras},
   language={Russian, with English summary},
   journal={Vests\=\i\ Akad. Navuk BSSR Ser. F\=\i z.-Mat. Navuk},
   date={1986},
   number={5},
   pages={11--15, 123},
   issn={0002-3574},
   %review={\MR{876665 (88d:17013)}},
}
\bib{Pre86-2}{article}{
   author={Premet, A. A.},
   title={Lie algebras without strong degeneration},
   language={Russian},
   journal={Mat. Sb. (N.S.)},
   volume={129(171)},
   date={1986},
   number={1},
   pages={140--153},
   issn={0368-8666},
   %review={\MR{830100 (87g:17018)}},
}		
\bib{Rob12}{book}{
   author={Roberts, K.},
   title={Lie Algebras and Incidence Geometry},
   school={PhD thesis, University of Birmingham},
   date={2012},
}

\bib{Ro10}{book}{
   author={Roozemond, Dan},
   title={Algorithms for Lie algebras of algebraic groups},
   school={PhD thesis, Technische Universiteit Eindhoven},
   date={2010},
}
\bib{Ro11}{article}{
   author={Roozemond, Dan},
   title={On Lie algebras generated by few extremal elements},
   journal={J. Algebra},
   volume={348},
   date={2011},
   pages={462--476},
   issn={0021-8693},
   %review={\MR{2852252}},
   %doi={10.1016/j.jalgebra.2011.10.015},
}
\bib{SvM13}{article}{
   author={Schillewaert, J.},
   author={Van Maldeghem, H.},
   title={Quadric Veronesean caps},
   journal={Bull. Belg. Math. Soc. Simon Stevin},
   volume={20},
   date={2013},
   number={1},
   pages={19--25},
   issn={1370-1444},
   %review={\MR{3082740}},
}
\bib{Spr98}{book}{
   author={Springer, T. A.},
   title={Linear algebraic groups},
   series={Progress in Mathematics},
   volume={9},
   edition={2},
   publisher={Birkh\"auser Boston, Inc., Boston, MA},
   date={1998},
   pages={xiv+334},
   isbn={0-8176-4021-5},
   %review={\MR{1642713 (99h:20075)}},
   %doi={10.1007/978-0-8176-4840-4},
}
\bib{Stb61}{article}{
   author={Steinberg, Robert},
   title={Automorphisms of classical Lie algebras},
   journal={Pacific J. Math.},
   volume={11},
   date={1961},
   pages={1119--1129},
   issn={0030-8730},
   %review={\MR{0143845 (26 \#1395)}},
}
\bib{Str04}{book}{
   author={Strade, Helmut},
   title={Simple Lie algebras over fields of positive characteristic. I},
   series={de Gruyter Expositions in Mathematics},
   volume={38},
   note={Structure theory},
   publisher={Walter de Gruyter \& Co., Berlin},
   date={2004},
   pages={viii+540},
   isbn={3-11-014211-2},
   %review={\MR{2059133 (2005c:17025)}},
   %doi={10.1515/9783110197945},
}
\bib{Str09}{book}{
   author={Strade, Helmut},
   title={Simple Lie algebras over fields of positive characteristic. II},
   series={de Gruyter Expositions in Mathematics},
   volume={42},
   note={Classifying the absolute toral rank two case},
   publisher={Walter de Gruyter \& Co., Berlin},
   date={2009},
   pages={vi+385},
   isbn={978-3-11-019701-3},
   %review={\MR{2573283 (2011c:17035)}},
   %doi={10.1515/9783110203059},
}
\bib{Str13}{book}{
   author={Strade, Helmut},
   title={Simple Lie algebras over fields of positive characteristic. III},
   series={de Gruyter Expositions in Mathematics},
   volume={57},
   note={Completion of the classification},
   publisher={Walter de Gruyter GmbH \& Co. KG, Berlin},
   date={2013},
   pages={x+239},
   isbn={978-3-11-026298-8},
   isbn={978-3-11-026301-5},
   %review={\MR{3025870}},
}
\bib{TVM04}{article}{
   author={Thas, J. A.},
   author={Van Maldeghem, H.},
   title={Full embeddings of the finite dual split Cayley hexagons},
   journal={Combinatorica},
   volume={24},
   date={2004},
   number={4},
   pages={681--698},
   issn={0209-9683},
   %review={\MR{2096821 (2005h:51007)}},
   %doi={10.1007/s00493-004-0041-8},
}


\bib{Tits66}{article}{
    AUTHOR = {Tits, J.},
     TITLE = {Sur les constantes de structure et le th\'eor\`eme d'existence des
              alg\`ebres de {L}ie semi-simples},
   JOURNAL = {Inst. Hautes \'Etudes Sci. Publ. Math.},
  FJOURNAL = {Institut des Hautes \'Etudes Scientifiques. Publications
              Math\'ematiques},
    NUMBER = {31},
      YEAR = {1966},
     PAGES = {21--58},
%      ISSN = {0073-8301},
%   MRCLASS = {17.30},
%  MRNUMBER = {0214638},
%MRREVIEWER = {W. Klingenberg},
%       URL = {http://www.numdam.org/item?id=PMIHES_1966__31__21_0},
}


\bib{Ti74}{book}{
   author={Tits, Jacques},
   title={Buildings of spherical type and finite BN-pairs},
   series={Lecture Notes in Mathematics, Vol. 386},
   publisher={Springer-Verlag, Berlin-New York},
   date={1974},
   pages={x+299},
   %review={\MR{0470099 (57 \#9866)}},
}


\bib{TW02}{book}{
   author={Tits, J.},
   author={Weiss, R. M.},
   title={Moufang polygons},
   series={Springer Monographs in Mathematics},
   publisher={Springer-Verlag, Berlin},
   date={2002},
   pages={x+535},
   isbn={3-540-43714-2},
   %review={\MR{1938841}},
   %doi={10.1007/978-3-662-04689-0},
}


\bib{Voe89}{article}{
   author={V{\"o}lklein, H.},
   title={On the geometry of the adjoint representation of a Chevalley
   group},
   journal={J. Algebra},
   volume={127},
   date={1989},
   number={1},
   pages={139--154},
   issn={0021-8693},
   %review={\MR{1029408 (91e:20033b)}},
   %doi={10.1016/0021-8693(89)90279-2},
}
\bib{Wei03}{book}{
   author={Weiss, R. M.},
   title={The structure of spherical buildings},
   publisher={Princeton University Press, Princeton, NJ},
   date={2003},
   pages={xiv+135},
   isbn={0-691-11733-0},
   %review={\MR{2034361 (2005b:51027)}},
}
\bib{Wei09}{book}{
   author={Weiss, R. M.},
   title={The structure of affine buildings},
   series={Annals of Mathematics Studies},
   volume={168},
   publisher={Princeton University Press, Princeton, NJ},
   date={2009},
   pages={xii+368},
   isbn={978-0-691-13881-7},
   %review={\MR{2468338 (2009m:51022)}},
}
\end{biblist}
\end{bibdiv}


